MetaBox+: A new Region Based Active Learning Method for Semantic Segmentation using Priority Maps

We present a novel region based active learning method for semantic image segmentation, called MetaBox+. For acquisition, we train a meta regression model to estimate the segment-wise Intersection over Union (IoU) of each predicted segment of unlabeled images. This can be understood as an estimation of segment-wise prediction quality. Queried regions are supposed to minimize to competing targets, i.e., low predicted IoU values / segmentation quality and low estimated annotation costs. For estimating the latter we propose a simple but practical method for annotation cost estimation. We compare our method to entropy based methods, where we consider the entropy as uncertainty of the prediction. The comparison and analysis of the results provide insights into annotation costs as well as robustness and variance of the methods. Numerical experiments conducted with two different networks on the Cityscapes dataset clearly demonstrate a reduction of annotation effort compared to random acquisition. Noteworthily, we achieve 95%of the mean Intersection over Union (mIoU), using MetaBox+ compared to when training with the full dataset, with only 10.47% / 32.01% annotation effort for the two networks, respectively.

==> _from_temlate.tex <==




% -------------------------------------------------------------- from template 
% @book{kn:Golub89,
%     author = "Golub, G.H. and {Van Loan}, C.F.",
%     title = "Matrix Computations",
%     edition = "2nd",
%     publisher = "Johns Hopkins University Press",
%     address = "Baltimore",
%     year = "1989",
%     kwds = "la"
% }

% @book{kn:deCarlini91,
%     author = "{de Carlini}, U. and Villano, U.",
%     title = "Transputers and parallel architectures -- message-passing
%               distributed systems",
%     publisher = "Ellis Horwood",
%     address = "Chichester",
%     year = "1991",
%     kwds = "par, arch, trans"
% }

% @book{kn:Modi88,
%     author = "Modi, J.J.",
%     title = "Parallel Algorithms and Matrix Computation",
%     publisher = "Oxford University Press",
%     address = "Oxford",
%     year = "1988",
%     kwds = "par, la"
% }

% @book{kn:Smith85,
%     author = "Smith, G.D.",
%     title = "Numerical Solution of Partial Differential Equations:
%               Finite Difference Methods",
%     edition = "3rd",
%     publisher = "Oxford University Press",
%     address = "Oxford",
%     year = "1985",
%     kwds = "pde"
% }

% @book{kn:Schofield89,
%     author = "Schofield, C.F.",
%     title = "Optimising {FORTRAN} programs",
%     publisher = "Ellis Horwood Publishing",
%     address = "Chichester",
%     year = "1989",
%     kwds = "lang, for"
% }

% @inbook{kn:daCunha92a,
%     author = "{da Cunha}, R.D. and Hopkins, T.R.",
%     title = "The Parallel Solution of Systems of Linear Equations using
%               Iterative Methods on Transputer Networks",
%     series = "Transputing for Numerical and Neural Network Applications",
%     pages = "1-13",
%     publisher = "IOS Press",
%     address = "Amsterdam",
%     year = "1992",
%     note = "Also as Report No. 16/92, Computing Laboratory, University of Kent at Canterbury, U.K.",
%     kwds = "par, iter"
% }

% @inbook{kn:daCunha92b,
%     author = "{da Cunha}, R.D. and Hopkins, T.R.",
%     title = "The Parallel Solution of Partial Differential Equations
%               on Transputer Networks",
%     series = "Transputing for Numerical and Neural Network Applications",
%     pages = "96-109",
%     publisher = "IOS Press",
%     address = "Amsterdam",
%     year = "1992",
%     note = "Also as Report No. 17/92, Computing Laboratory, University of Kent at Canterbury, U.K.",
%     kwds = "par, pde"
% }

% @misc{kn:Atkin,
%     author = "Atkin, P.",
%     title = "Performance Maximisation",
%     howpublished = "INMOS Technical Note 17",
%     kwds = "perf, trans, loop"
% }

% @article{kn:Saad85,
%     author = "Saad, Y.",
%     title = "Practical use of polynomial preconditionings for the
%               {Conjugate Gradient} method",
%     journal = "SIAM Journal of Scientific and Statistical Computing",
%     volume = "6",
%     pages = "865-881",
%     year = "1985",
%     kwds = "cg, precon, poly"
% }

% @article{kn:Eisenstat81,
%     author = "Eisenstat, S.C.",
%     title = "Efficient implementation of a class of preconditioned 
%               {Conjugate Gradient} methods",
%     journal = "SIAM Journal of Scientific and Statistical Computing",
%     volume = "2",
%     pages = "1-4",
%     year = "1981",
%     kwds = "cg, precon"
% }

% @article{kn:Adams85,
%     author = "Adams, L.",
%     title = "{m-Step} preconditioned {Gradient} methods",
%     journal = "SIAM Journal of Scientific and Statistical Computing",
%     volume = "6",
%     pages = "452-463",
%     year = "1985",
%     kwds = "cg, precon, poly"
% }

% @article{kn:Johnson83,
%     author = "Johnson, O.G. and Micchelli, C.A. and Paul, G.",
%     title = "Polynomial preconditioners for {Conjugate Gradient} 
%               calculations",
%     journal = "SIAM Journal of Numerical Analysis",
%     volume = "20",
%     pages = "362-376",
%     year = "1983",
%     kwds = "cg, precon, poly"
% }


==> notation.tex <==
% Update 20.05.2020 10:45 Pascal 

%--------------------------------------------------------------------------------------------------------
% Index  
%--------------------------------------------------------------------------------------------------------
% ij                      position image/prediction/...
% k                       sample
% l                       selected box


%--------------------------------------------------------------------------------------------------------
% Variable
%--------------------------------------------------------------------------------------------------------
% m_{init, meta, al}      number samples in initialisation, for MetaSeg, in each AL iteration
% n                       number of classes
% h                       sample height 
% w                       sample wide
% b_{size}                box-side length
% p                       p-quantile 
% t                       type of f,g (see below)
%
% H                       Entropy (image)
% M                       MetaSeg (image)
% C                       Cost (Image) (given)
% \hat{C}                 Cost (Image) estimated 
% $\delta$                Threshold for the IoU of pseudo labels


%--------------------------------------------------------------------------------------------------------
% Sets
%--------------------------------------------------------------------------------------------------------
% \mathcal{P}             data pool (Cityscapes train set)
% \mathcal{U}             Unlabeled data
% \mathcal{L}             Labeled data
% \mathcal{M}             MetaSeg (training's)data
% \mathcal{\hat{L}}       Pseudo-Labels data 

%--------------------------------------------------------------------------------------------------------
% Functions
%--------------------------------------------------------------------------------------------------------
% f                       getting information image
% g                       getting information map
% h                       getting query map with fusion 


%--------------------------------------------------------------------------------------------------------
% Convention
%--------------------------------------------------------------------------------------------------------
% ^{ Index }              Index e.g. sample, selected box 
% _{ type }               type, e.g. in number samples or in function (image, map, fusion) 



%--------------------------------------------------------------------------------------------------------
% Various stuff
%--------------------------------------------------------------------------------------------------------
% Q_p                      p-quantile (in normalization)
% cost_{}                 cost metrics based c_{...}^{..}, see sec 4.1


%--------------------------------------------------------------------------------------------------------
% Open Questions: finde die angemessene Abstraktionsebene 
%--------------------------------------------------------------------------------------------------------
% Die Unterteilung der Datenmengen (sets) wäre noch möglich: img, gt, pred, seg, pseudo, clicks wobei alle die gleiche Grö0e (w,h) hätten. Werte die nicht angegeben sind könnte man auf NULL oder 255 (ignore) setzen. So hätte man eine einheitliche Datenstruktur. 

% Das CNN und MetaSeg Modell könnte man auch mit einer Abbildung (\phi o.ä.) bezeichnen. 
